Complex Neural Network based Joint AoA and AoD Estimation for Bistatic ISAC

Integrated sensing and communication (ISAC) in wireless systems has emerged as a promising paradigm, offering the potential for improved performance, efficient resource utilization, and mutually beneficial interactions between radar sensing and wireless communications, thereby shaping the future of wireless technologies. In this work, we present two novel methods to address the joint angle of arrival and angle of departure estimation problem for bistatic ISAC systems. Our proposed methods consist of a deep learning (DL) solution leveraging complex neural networks, in addition to a parameterized algorithm. By exploiting the estimated channel matrix and incorporating a preprocessing step consisting of a coarse timing estimation, we are able to notably reduce the input size and improve the computational efficiency. In our findings, we emphasize the remarkable potential of our DL-based approach, which demonstrates comparable performance to the parameterized method that explicitly exploits the multiple-input multiple-output (MIMO) model, while exhibiting significantly lower computational complexity.

==> Actions/ARP-contribution.tex <==
\textbf{Antenna radiation pattern impact.}
We explore how the antenna radiation pattern influences the overall performance of the bi-static \ac{ISAC} system. 
 Following the introduction of antenna radiation patterns to the system model, we analyze the behavior of the \ac{CRB} by varying parameters associated with the antenna radiation pattern.

==> Actions/list-of-contributions.tex <==
\begin{itemize}
	\item \textbf{Novel joint \ac{AoA}/\ac{AoD} \ac{DL} estimator.} We present a new \ac{DL} technique for sensing parameter estimation, i.e. the \acp{AoA} and \acp{AoD} in an \ac{ISAC} system. 
	Departing from conventional input sources, the method utilizes the estimated channel matrix, which captures essential information regarding the sensing parameters. 
	The \ac{DL} model employs complex-valued neural networks, and includes complex convolutional and linear layers, with weights represented as complex matrices, enhancing the model's ability to accurately represent the channel matrix. The complex rectified linear unit (CReLU) is chosen as the activation function. 
	The network structure comprises three hidden layers and a final output layer predicting the sensing parameters. Moreover, the \ac{MSE} serves as the objective function during the training phase.
	
	\item \textbf{Novel design of a parameterized \ac{AoA}/\ac{AoD} estimator.} We develop a parameterized method for \ac{AoA}/\ac{AoD} estimator, which exploits the complete model knowledge, including the array geometries. 
	The method involves transforming the received channel matrix by leveraging the \ac{ULA} structures at transmit and receive sides into smaller channel matrices with given sub-array sizes.
	The method makes use of the induced Hankel structure to further compute certain eigenvalues, which aid in the \ac{AoD} estimation. 
	Regarding \ac{AoA} estimation, a \ac{LS} fit is required at a later stage of the algorithm. 
	
	
	\item \textbf{Presentation of maximum likelihood and \ac{CRB}.} In order to assess the performance of our proposed estimators, it is essential to showcase the maximum likelihood criterion for the estimation problem at hand, in addition to the \ac{CRB} for benchmarking purposes.
	
	\item \textbf{Comprehensive computational complexity analysis.} We provide a complexity analysis of the two proposed methods, with a focus on the total number of multiplications and additions. 
	We detail the various complexities involved in the \ac{DL} technique, which utilizes architectures with three hidden layers by counting the complexities involved in its different operations.
	For the parametrized approach, we provide a breakdown of computational complexities associated with specific blocks, including channel estimation, coarse timing estimation, and sensing estimation, highlighting the required estimation overheads and the total number of operations for each block. 
	Additionally, a comparison of the computational complexities between the proposed 2D parameterized algorithm and the \ac{MLE} method is presented in terms of additional and multiplication operations.
	
	\item \textcolor{black}{\input{Actions/ARP-contribution.tex}}

\end{itemize}

%\begin{itemize}
%    \item Development of a new \ac{DL} technique to estimate the \ac{AoA} and \ac{AoD}. This method also provides an estimation of the number of targets with indistinguishable delays.
%    \item Design of a parameterized-based method that uses full knowledge of the model for \ac{AoA} and \ac{AoD} estimation, i.e. the algorithm exploits the known array geometry. 
%    \item Presentation of the maximum likelihood criterion and \ac{CRB}.
%    \item Evaluation of different training strategies based on a \ac{SNR} analysis.
%    \item Complexity analysis of both proposed methods in terms of the number of multiplications and additions.
%    \item Performance comparison in terms of \ac{MSE} and complexity between the \ac{DL}-based estimation method and the parameterized-based method.
%\end{itemize}

==> Actions/list-of-insights.tex <==
Furthermore, we unveil some important insights, i.e.
\begin{itemize}
	\item 
	Through simulations, we study the impact of training \ac{SNR} on the achieved \ac{MSE} performance. 
	More specifically, the \ac{MLP} architecture is trained using simulation data generated at specific \acp{SNR}, and the network's performance is evaluated on a test dataset spanning a range of given \ac{SNR} values.
	We observe that loss curves steadily decrease during training, indicating effective learning and generalization to unseen data. 
	Regarding overfitting, we employ a learning rate schedule.
	In addition, we showcase various simulation results illustrating the superior performance and potential of the proposed methods compared, and their closeness to the \ac{CRB} benchmarks. 
	

	\item In terms of computational complexities, our simulations show that the proposed \ac{DL} technique enjoys less computational complexity compared to the parametric $2$D estimation algorithm. For instance, with $8$ receive antennas, the $2$D algorithm requires $6.5$ times more multiplications than the \ac{DL} one, which is $15.27$\% of the computational complexity required by the $2$D algorithm for multiplications. Despite a performance degradation, particularly at higher \ac{SNR} values, these results underscore the substantial percentage gains in computational efficiency and scalability offered by the \ac{DL} architecture.
\end{itemize}

%    \item Evaluation of different training strategies based on a \ac{SNR} analysis.
%    \item Performance comparison in terms of \ac{MSE} and complexity between the \ac{DL}-based estimation method and the parameterized-based method.

==> Actions/summary-of-actions.tex <==
In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
	\item We have indicated that \ac{ISAC} approach here is a communication-assisted sensing one, where communication signals sent by a \ac{BS} are exploited for finely estimating target sensing parameters in a bi-static setting. Additionally, the integration involves leveraging preamble knowledge from communication standards for efficient sensing tasks.
	\item We have better elaborated on the contributions.
	\item To ensure the duplicability of our work, we have provided both the simulated dataset and code on {\tt{GitHub}}, along with the corresponding link for easy access.
	
	\item We have explained the underperformance of the NN-based approach, relative to parameter estimation, appearing in Fig. 7 of the initial submission (Fig. \ref{fig_2TarPerPeak} of the revised manuscript).
	\item We have acknowledged that the channel and timing estimation techniques are indeed classical and we have mentioned the motivation behind using classical ones.
	\item We have highlighted the reason behind the non-monotonic behaviour of the MSE results appearing in Fig. 4 (Fig. \ref{fig_snr_analysis} in the updated manuscript)
	\item We have clarified the gains of the proposed technique when compared to brute force MLE, and we have generated a figure to highlight those gains. 
	\item We have further clarified the required estimation overheads.
	\item We have mentioned and explained that the approach followed in this paper is not only limited to \ac{OFDM}.
	\item We have indicated that the scenario necessitates reapplying the proposed technique when angles change in the assumed scenario and that future related work will address and propose tracking techniques for the underlying scenario.

	\item We have generalized the work to a general antenna radiation pattern setting and added new simulations in order to show the impact of antenna radiation patterns.
	\item We have explained symbols appearing within the manuscript.
	\item We have corrected typos that were appearing in the first submission.
\end{itemize}



==> Actions2/summary-of-actions2.tex <==
In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
	\item Upon revisiting Section \ref{sec:introduction}, we have made changes to the contributions to better elucidate the unique contributions of our work. 
\end{itemize}



==> Response/R1C1.tex <==
The authors would like to thank the reviewer for the comment.
% three main scenarios: comm assisted, Radar-ass, Joint
The \ac{ISAC} framework can be broadly categorized into three categories: communication-centric, radar-centric, and joint design \cite{9540344}, \cite{10038611}. In communication-centric, which is the main focus of this paper, radar sensing can be considered as an "add-on" to a communication system. The primary objective of this design approach is to leverage communication waveforms to discern radar information via the analysis of target echoes. In radar-centric, however, the approach modulates information signaling within established radar waveforms, like chirping \cite{9828505}. The joint design covers systems that are collaboratively designed from the outset to provide an adjustable balance between sensing and communication performance \cite{10061453}, \cite{8386661}. 
Following a communication-centric approach, our approach involves a communication signal sent to each user by a \ac{BS}, primarily dedicated to communication tasks. The radar receiver then utilizes the backscattered communication signal for precise estimation of target sensing parameters.
%In addition, we would also like to draw attention to a mono-static setting described in \cite{10279367} for \ac{OTFS} signaling within the \ac{ISAC} framework. Additionally, in the work presented in \cite{10250200}, a \ac{TDD} massive \ac{MIMO} system was employed, with the \ac{BS} serving communication users while concurrently leveraging the scattered signal for environmental sensing.
Moreover, the scenario herein, involving communication-centric sensing, within the \ac{ISAC} framework, considers the interaction between radar and \ac{BS}, as the former is making use of the protocol followed by the latter in terms of knowledge of the preamble. It is also worth mentioning some references that use \ac{ISAC} communication-assisted sensing. For example, \cite{10279367} leverages \ac{OTFS} signaling within \ac{ISAC} to perform communication-assisted sensing by making use of the echo signals to sense a target. Furthermore, \cite{10250200} utilizes a \ac{TDD} massive \ac{MIMO} system, whereby the \ac{BS} serving multiple communication users and simultaneously utilizing the echo signal for environmental sensing.
Moreover, our approach incorporates preamble knowledge based on communication standards to perform estimation sensing tasks, which can further enable \ac{ISAC} applications.
Hence, the proposed system is a communication-assisted sensing system where the main interest lies in MSE of target \acp{AoA} rather than the communication performance.

==> Response/R2C1.tex <==
The authors would like to thank the reviewer for the comment.
Yes, indeed, both are classical approaches, especially for communication tasks.
For example, the channel estimation in equation \eqref{eq:method2_step0} of the updated manuscript is the well-known \ac{LS} channel estimation.
Our aim, then, is to show that sensing can also be accomplished using some familiar preprocessing techniques, which are quite known to the community and are also easy to implement.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
